Mainlining Databases: Supporting Fast Transactional Workloads on Universal Columnar Data File Formats

The proliferation of modern data processing tools has given rise to open-source columnar data formats. The advantage of these formats is that they help organizations avoid repeatedly converting data to a new format for each application. These formats, however, are read-only, and organizations must use a heavy-weight transformation process to load data from on-line transactional processing (OLTP) systems. We aim to reduce or even eliminate this process by developing a storage architecture for in-memory database management systems (DBMSs) that is aware of the eventual usage of its data and emits columnar storage blocks in a universal open-source format. We introduce relaxations to common analytical data formats to efficiently update records and rely on a lightweight transformation process to convert blocks to a read-optimized layout when they are cold. We also describe how to access data from third-party analytical tools with minimal serialization overhead. To evaluate our work, we implemented our storage engine based on the Apache Arrow format and integrated it into the DB-X DBMS. Our experiments show that our approach achieves comparable performance with dedicated OLTP DBMSs while enabling orders-of-magnitude faster data exports to external data science and machine learning tools than existing methods.

==> Makefile <==
# Makefile for LaTeX files

LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

PDFPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.pdf$$/) { print "$$foo[2] "; } else { print "$$foo[2].pdf "; }}' *.tex)
DEP	= *.tex scripts/plots.py

TRG	= $(SRC:%.tex=%.pdf)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false


all 	: $(TRG)

define run-latex
	  $(COPY);$(LATEX) $<
	  egrep -q $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	  egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	  egrep -q $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) ; true
	  egrep -q $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) ; true
	  if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	  $(RM) $(<:%.tex=%.toc.bak)
	  # Display relevant warnings
	  egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

$(TRG)	: %.pdf : %.tex $(DEP) $(PDFPICS) $(BIBFILE)
	  @$(run-latex)

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.pdf=%.aux) $(TRG:%.pdf=%.bbl) $(TRG:%.pdf=%.blg) $(TRG:%.pdf=%.log) $(TRG:%.pdf=%.out) $(TRG:%.pdf=%.dvi) $(TRG:%.pdf=%.synctex.gz)

.PHONY	: all show clean ps pdf showps stylecheck spellcheck

figures:
	echo "Generating plots..."
	python scripts/plots.py

view:
	acroread $(PDF)

osx:
	open $(PDF)

combined:
	pdfunite cover.pdf storage.pdf combined.pdf

# Check style:
stylecheck:
	printf "weasel words: "
	sh ./scripts/weasel *.tex
	printf "\npassive voice: "
	sh ./scripts/passive *.tex
	printf "\nduplicates: "
	perl ./scripts/dups *.tex
	printf "\ndone\n"

# Check spelling with aspell
spellcheck:
	find . -name "*.tex" -exec aspell --lang=en --mode=tex --dont-suggest --personal=./.aspell.en.pws check "{}" \;

######################################################################
# Define rules for PDF source files.
%.pdf: %.eps
	epstopdf $< > $(<:%.eps=%.pdf)


==> tags <==
!_TAG_FILE_SORTED	2	/0=unsorted, 1=sorted, 2=foldcase/
BASEDIR	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^BASEDIR = os.path.dirname(os.path.realpath(__file__))$/;"	v	language:Python
BIBFILE	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^BIBFILE := $(shell perl -ne '($$_)=\/^[^%]*\\\\bibliography\\{(.*?)\\}\/;@_=split \/,\/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))$/;"	m	language:Make
BIBTEX	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^BIBTEX	= bibtex$/;"	m	language:Make
COPY	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi $/;"	m	language:Make
DEP	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^DEP	= *.tex scripts\/plots.py$/;"	m	language:Make
GROUP_X_TICK_LABELS	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^GROUP_X_TICK_LABELS = ["", "0", "2", "4", "8", "16", "32", "64", "128", "256", ""]$/;"	v	language:Python
GROUP_X_VALUES	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^GROUP_X_VALUES = [[0, 1, 2, 3, 4, 5, 6, 7, 8, 9, 10]]$/;"	v	language:Python
HATCHES	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^HATCHES = ['\/\/', 'O', '\\\\', 'x', '\/', '\\\\\\\\']$/;"	v	language:Python
label_helper	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def label_helper(labels):$/;"	f	language:Python
LATEX	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^LATEX	= pdflatex$/;"	m	language:Make
main	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def main():$/;"	f	language:Python
MAKEIDX	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^MAKEIDX = "^[^%]*\\\\makeindex"$/;"	m	language:Make
MAKEINDEX	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^MAKEINDEX = makeindex$/;"	m	language:Make
MARKERS	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^MARKERS = ['o', 's', '<', 'v', 'p', '^', '>', 'D']$/;"	v	language:Python
matplotlib	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^import matplotlib.lines as mlines$/;"	i	language:Python
matplotlib	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^import matplotlib.patches as mpatches$/;"	i	language:Python
matplotlib	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^import matplotlib.pyplot as plt$/;"	i	language:Python
MaxNLocator	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^from matplotlib.ticker import MaxNLocator$/;"	i	language:Python
mlines	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^import matplotlib.lines as mlines$/;"	i	language:Python
mpatches	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^import matplotlib.patches as mpatches$/;"	i	language:Python
MPRINT	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^MPRINT = "^[^%]*print"$/;"	m	language:Make
MT_X_TICK_LABELS	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^MT_X_TICK_LABELS = [""] + [str(i) if i % 5 == 0 or i == 1 else "" for i in range(1, 21)] + [""]$/;"	v	language:Python
MT_X_VALUES	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^MT_X_VALUES = [range(22)]$/;"	v	language:Python
np	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^import numpy as np$/;"	i	language:Python
OPT_CONTEXT	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^OPT_CONTEXT   = "notebook"$/;"	v	language:Python
OPT_FONT_SIZE	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^OPT_FONT_SIZE = 2.0$/;"	v	language:Python
OPT_HEIGHT	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^OPT_HEIGHT    = 4.$/;"	v	language:Python
OPT_STYLE	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^OPT_STYLE     = "whitegrid"$/;"	v	language:Python
OPT_WIDTH	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^OPT_WIDTH     = 8.$/;"	v	language:Python
os	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^import sys, os.path$/;"	i	language:Python
OUTDATED	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^OUTDATED = echo "EPS-file is out-of-date!" && false$/;"	m	language:Make
path	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^import sys, os.path$/;"	i	language:Python
PDFPICS	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^PDFPICS := $(shell perl -ne '@foo=\/^[^%]*\\\\(includegraphics)(\\[.*?\\])?\\{(.*?)\\}\/g;if (defined($$foo[2])) { if ($$foo[2] =~ \/.pdf$$\/) { print "$$foo[2] "; } else { print "$$foo[2].pdf "; }}' *.tex)$/;"	m	language:Make
plot_all_group_sensitivity	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_all_group_sensitivity(save=False):$/;"	f	language:Python
plot_all_mt	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_all_mt(save=False):$/;"	f	language:Python
plot_all_vector_sensitivity	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_all_vector_sensitivity(save=False):$/;"	f	language:Python
plot_bar_graph	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_bar_graph(y_values, $/;"	f	language:Python
plot_line_graph	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_line_graph(x_values,$/;"	f	language:Python
plot_q1	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q1():$/;"	f	language:Python
plot_q13	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q13(save=False):$/;"	f	language:Python
plot_q13_group_sensitivity	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q13_group_sensitivity(save=False):$/;"	f	language:Python
plot_q13_vector_sensitivity	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q13_vector_sensitivity(save=False):$/;"	f	language:Python
plot_q14	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q14(save=False):$/;"	f	language:Python
plot_q14_group_sensitivity	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q14_group_sensitivity(save=False):$/;"	f	language:Python
plot_q14_vector_sensitivity	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q14_vector_sensitivity(save=False):$/;"	f	language:Python
plot_q19	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q19(save=False):$/;"	f	language:Python
plot_q19_group_sensitivity	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q19_group_sensitivity(save=False):$/;"	f	language:Python
plot_q19_vector_sensitivity	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q19_vector_sensitivity(save=False):$/;"	f	language:Python
plot_q1_group_sensitivity	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q1_group_sensitivity(save=False):$/;"	f	language:Python
plot_q1_vector_sensitivity	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q1_vector_sensitivity(save=False):$/;"	f	language:Python
plot_q3	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q3():$/;"	f	language:Python
plot_q3_group_sensitivity	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q3_group_sensitivity(save=False):$/;"	f	language:Python
plot_q3_vector_sensitivity	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_q3_vector_sensitivity(save=False):$/;"	f	language:Python
plot_simd_filter_micro	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_simd_filter_micro(save=False):$/;"	f	language:Python
plot_simd_filter_micro_legend	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_simd_filter_micro_legend():$/;"	f	language:Python
plot_simd_probe	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_simd_probe():$/;"	f	language:Python
plot_simd_probe2	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_simd_probe2(save=False):$/;"	f	language:Python
plot_simd_probe_dev4	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_simd_probe_dev4(save=False):$/;"	f	language:Python
plot_stacked_bar_graph	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_stacked_bar_graph(y_values,$/;"	f	language:Python
plot_tpch_all	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_tpch_all(save=False):$/;"	f	language:Python
plot_tpch_all_legend	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_tpch_all_legend(save=False):$/;"	f	language:Python
plot_tw	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_tw(save=False):$/;"	f	language:Python
plot_vw_hyper	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^def plot_vw_hyper(save=False):$/;"	f	language:Python
plt	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^import matplotlib.pyplot as plt$/;"	i	language:Python
RERUN	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"$/;"	m	language:Make
RERUNBIB	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^RERUNBIB = "No file.*\\.bbl|Citation.*undefined"$/;"	m	language:Make
RM	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^RM = rm -f$/;"	m	language:Make
run-latex	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^define run-latex$/;"	m	language:Make
SAVEDIR	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^SAVEDIR = os.path.join(BASEDIR, "figures")$/;"	v	language:Python
SELECTIVITY_X_TICK_LABELS	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^SELECTIVITY_X_TICK_LABELS = [""] + [str(float(i)\/10) if i % 2 == 0 else "" for i in range(0, 11)] + [""]$/;"	v	language:Python
SELECTIVITY_X_VALUES	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^SELECTIVITY_X_VALUES = [range(13)]$/;"	v	language:Python
sns	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^import seaborn as sns$/;"	i	language:Python
SRC	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^SRC	:= $(shell egrep -l '^[^%]*\\\\begin\\{document\\}' *.tex)$/;"	m	language:Make
sys	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^import sys, os.path$/;"	i	language:Python
TRG	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^TRG	= $(SRC:%.tex=%.pdf)$/;"	m	language:Make
USETHUMBS	/Users/Tianyu/Desktop/peloton-pubs/storage-arrow/Makefile	/^USETHUMBS = "^[^%]*thumbpdf"$/;"	m	language:Make
VECTOR_X_TICK_LABELS	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^VECTOR_X_TICK_LABELS = ["", "64", "", "256", "", "1K", "", "4K", "", "16K", "", "64K", "", "256K", ""]$/;"	v	language:Python
VECTOR_X_VALUES	/Users/Tianyu/Desktop/peloton-pubs/querycomp-rof/scripts/plots.py	/^VECTOR_X_VALUES = [[0, 1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14]]$/;"	v	language:Python

